Active Learning over DNN: Automated Engineering Design Optimization for Fluid Dynamics Based on Self-Simulated Dataset

Optimizing fluid-dynamic performance is an important engineering task. Traditionally, experts design shapes based on empirical estimations and verify them through expensive experiments. This costly process, both in terms of time and space, may only explore a limited number of shapes and lead to sub-optimal designs. In this research, a test-proven deep learning architecture is applied to predict the performance under various restrictions and search for better shapes by optimizing the learned prediction function. The major challenge is the vast amount of data points Deep Neural Network (DNN) demands, which is improvident to simulate. To remedy this drawback, a Frequentist active learning is used to explore regions of the output space that DNN predicts promising. This operation reduces the number of data samples demanded from ~8000 to 625. The final stage, a user interface, made the model capable of optimizing with given user input of minimum area and viscosity. Flood fill is used to define a boundary area function so that the optimal shape does not bypass the minimum area. Stochastic Gradient Langevin Dynamics (SGLD) is employed to make sure the ultimate shape is optimized while circumventing the required area. Jointly, shapes with extremely low drags are found explored by a practical user interface with no human domain knowledge and modest computation overhead.

==> old.tex <==
\textbf{Claim 1}: $\forall P \in \Bc$ except a set that is nowhere dense, $\forall C \in \Bc(P)$, there is an open set around $C$ that contains no element in $\Bc(P)$ except $C$ itself. 

% To prove that it is nowhere dense, we first observe that suppose we have $P, C\neq I$ such that 
% \begin{align*}
%     C^T P C - P = 0 \numberthis\label{eq:singular_identity}
% \end{align*}

To prove this claim we pick any $P \in \Bc$ and $C \in \Bc(P)$, if this claim is false, there must exist a $D \in \mathbb{R}^{n \times n}$ that satisfy the following
\begin{enumerate}
    \item $D \neq 0$
    \item $D \oneb = 0$ (to ensure $C+\epsilon D \in \Cc$)
    \item For sufficiently small $\epsilon$, $(C + \epsilon D)^T P (C + \epsilon D) = C^T P C$
\end{enumerate}  
Suppose such a $D$ exists, we prove a contradiction. 


\begin{align*}
    (C+\epsilon D)^T P (C+\epsilon D) = C^TPC + \epsilon(D^TPC + C^TPD) + O(\epsilon^2) 
\end{align*}
Therefore for condition 3 to hold we must have
\[ D^T P C + C^T PD = 0 \]

Conjecture: rank of solution space for above equation must be independent of $C$ as long as $C$ has full rank.

Reason for conjecture: Numerically tried $P = \mathcal{N}(0, 1)$, $P=I$, $P=-I$, $P=\mathrm{abs}(\mathcal{N}(0, 1))$, $P=1$, and $C=\mathcal{N}(0, 1)$, $C=I$, $C=P$, $C=P^{-1}$, $C=P^T$, $C=-P$, and matrices from width 4-25, and in all these cases solution space rank of above equation is independent of $C$.

% To show this let $\mathcal{T}$ be the transpose operator $\mathbb{R}^{n \times n} \to \mathbb{R}^{n \times n}$, $\mathcal{I}$ be the identity operator, and let $\mathcal{C}^T, \mathcal{P}, \mathcal{P}^T$ be the operators that
% \begin{align*}
%     \mathcal{C}^T: &A \in \mathbb{R}^{n \times n} \to C^T A \\
%     \mathcal{P}: &A \in \mathbb{R}^{n \times n} \to PA \\
%     \mathcal{P}^T: &A \in \mathbb{R}^{n \times n} \to P^TA 
% \end{align*}
% Note that $\mathcal{T}$ is an invertible operator, while $\mathcal{C}^T, \mathcal{P}, \mathcal{P}^T$ are invertible if the corresponding matrix $C, P$ are invertible. Rewrite the above equation in operator form we have

% \begin{align*}
%     \mathcal{T} \circ \mathcal{C}^T \circ \mathcal{P}^T (D) + \mathcal{C}^T \circ \mathcal{P}(D) = (\mathcal{T} + \mathcal{I}) \circ \mathcal{C}^T \circ (\mathcal{P} + \mathcal{P}^T) (D) = 0
% \end{align*}

% Lemma (conjectured): If $A, B$ are full rank, the linear equality of $D$: $D^T A + BD = 0$ has non-zero solution $D \neq 0$ if and only if $A^T - B$  has all-zero columns. 

% \begin{proof}
% We vectorize $D$ to convert the equation from matrix equality vector equality. 
% \end{proof}

% Proof strategy: based on this lemma show that it is highly unlikely to have $(PC)^T=-C^TP$ for some columns, because this would imply P is anti-symmetric on some column/rows if it is full rank (C is full rank if P is). Show that insufficient rank or anti-symmetric matrices are nowhere dense. 
Because the proof holds for any $C$, we can pick the most convenient one. In particular, we can pick $C = I$. 

Conjecture: The equation $D^T P + PD$ has no solution $D\neq 0$, $D\oneb = 0$ for nowhere dense $P$

Reason for conjecture: Based on numerical simulations we have $D^T P + PD=0$ have no solution that satisfy $D\oneb = 0$ under random $P$. In particular the equality always have rank $n^2 - \lfloor n/2 \rfloor$, but under additional $n$ constraints $D \oneb = 0$ always have full rank.
% \begin{align*} 
% \frac{\partial C^T PC}{\partial c_{ij}} &= 
% \left( \begin{array}{ccc}
% \frac{\partial c_1^T P c_1}{c_{ij}} & \frac{\partial c_1^T P c_2}{c_{ij}} &  \cdots \\
% \frac{\partial c_2^T P c_1}{c_{ij}} & \frac{\partial c_2^T P c_2}{c_{ij}} &  \cdots \\
% \cdots & \cdots & \cdots 
% \end{array} \right) 
% = \left( \begin{array} {cccccc}
% &&  & \frac{\partial c_1^T P c_i}{\partial c_{ij}} && \\
% && & \frac{\partial c_2^T P c_i}{\partial c_{ij}} && \\
% \frac{\partial c_i^T P c_1}{\partial c_{ij}} & \frac{\partial c_i^T P c_2}{\partial c_{ij}} & \cdots & \frac{\partial c_i^T P c_i}{\partial c_{ij}} & \frac{\partial c_{i+1}^T P c_i}{\partial c_{ij}} & \cdots \\
% &&  & \frac{\partial c_{i+1}^T P c_i}{\partial c_{ij}} && \\
% &&  & \cdots &&
% \end{array} \right) 
% %+ \left( \begin{array} {ccccc}
% % && \frac{\partial c_1^T P c_i}{\partial c_{ij}} && \\
% % && \frac{\partial c_2^T P c_i}{\partial c_{ij}} && \\
% % 0 & \cdots & \cdots & \cdots & 0 \\
% % && \frac{\partial c_i^T P c_i}{\partial c_{ij}} && \\
% % && \cdots && 
% % \end{array} \right)
% \end{align*}
% We compute each of the derivatives in turn. Let $k \neq i$
% \begin{align*}
%     \frac{\partial c_i^T P c_k}{\partial c_{ij}} &= \frac{\partial \sum_{u, v} c_{iu}P_{uv}c_{kv}}{\partial c_{ij}} =  \sum_{v} P_{jv}c_{kv} = P_j c_k \\
%     \frac{\partial c_i^T P c_i}{\partial c_{ij}} &= \frac{\partial \sum_{u, v} c_{iu}P_{uv}c_{iv}}{\partial c_{ij}} = \sum_{v \neq j} P_{jv}c_{iv} + \sum_{u \neq j} c_{iu} P_{uj} + 2 P_{jj} c_{ij} = P_j c_i + C_i p_j \\
%     \frac{\partial c_k^T P c_i}{\partial c_{ij}} &= \frac{\partial \sum_{u, v} c_{ku}P_{uv}c_{iv}}{\partial c_{ij}} =  \sum_{u} c_{ku}P_{uj} = C_k p_j  \\
% \end{align*}
% Therefore the above derivative becomes 
% \begin{align*}
% \frac{\partial C^T PC}{\partial c_{ij}} =\left( \begin{array}{c} 0 \\ \cdots \\ P_j C \quad (i\mathrm{-th\ row}) \\ \cdots \\ 0 \end{array} \right) + \left( \begin{array}{ccccc} 0 & \cdots & C p_j & \cdots & 0 \\
% && (i\mathrm{-th\ column}) &&\end{array} \right) 
% \end{align*}
% For sufficiently small $\epsilon$ to satisfy  $(C + \epsilon D)^T P (C + \epsilon D) = C^T P C$ we must have 
% \[ \sum_{i, j} d_{ij} \frac{\partial C^T PC}{\partial c_{ij}}  = 0\]
% This means that we must have for all $i$
% \[ \sum_j d_{ij} P_j C = (\sum_j d_{ij} P_j) C = 0 \]
% If $P$ is full rank, $\lbrace P_j, 1 \leq j \leq n \rbrace$ must be linearly independent and we must have $\sum_j d_{ij} P_j \neq 0$, which means that $C$ cannot be full rank. Then $C^T P C $ cannot be full rank. This contradicts the fact that $C^TPC = P$. 

\textbf{Consequence of Claim 1}: the set of $P \in \Bc$ such that $\Bc(P)$ is not a countable set is nowhere dense. 

\textbf{Claim 2}: $\forall P \in \Bc$, $\forall C \in \Bc(P)$, there is an open set $\mathfrak{C}$ around $C$ such that in an open set $\mathfrak{P}$ around $P$,  such that the set of $P' \in \mathfrak{P}$ with $\Bc(P') \cap \mathfrak{C} \neq \emptyset$ is nowhere dense.

To prove this claim we consider small perturbations around $P$ and $C$: $P+ \epsilon \Delta P$, $C+\epsilon \Delta C$, we show that for all but a set of measure $0$, a perturbation $\epsilon \Delta P$ does not have a corresponding $\epsilon \Delta C$ that preserves the identity of Eq.(\ref{eq:singular_identity})
\begin{align*}
&(C+\epsilon \Delta C)^T(P+\epsilon \Delta P)C+\epsilon \Delta C) - P - \epsilon \Delta P \\\
&= (C^T P C - P) + \epsilon(\Delta C^T PC + C^T \Delta P C + C^T P \Delta C - \Delta P) + O(\epsilon^2)  \\
&= \epsilon(\Delta C^T PC + C^T \Delta P C + C^T P \Delta C - \Delta P) + O(\epsilon^2) = 0 
\end{align*}
To satisfy this for sufficiently small $\epsilon$ we must have
\[ \Delta C^T PC + C^T P \Delta C = \Delta P - C^T \Delta P C \]
But additionally we must have $\oneb^T \Delta P \oneb = 0$ and $\Delta C\oneb = 0$. For any given $C\neq I$, the set of $\Delta P$ such that $\Delta P - C^T \Delta P C$ is full rank has measure 1 (to be confirmed). Therefore, because 
\[ \dim \lspan(\Delta C^T PC + C^T P \Delta C) \leq n^2 - n \]
while 
\[ \dim \lspan(\Delta P - C^T \Delta P C) = n^2 - 1 \]
For all $\Delta P$ but a set of measure 0, the equation does not have a solution. 

\textbf{Consequence of Claim 2}: For any $P \in \Bc$ there is an open neighborhood of $P$ in which $\Bc$ is nowhere dense.
